Phase-field material point method for dynamic brittle fracture with isotropic and anisotropic surface energy

A novel phase field material point method is introduced for robust simulation of dynamic fracture in elastic media considering the most general case of anisotropic surface energy. Anisotropy is explicitly introduced through a properly defined crack density functional. The particular case of impact driven fracture is treated by employing a discrete field approach within the material point method setting. In this, the equations of motion and phase field governing equations are solved independently for each discrete field using a predictor-corrector algorithm. Contact at the interface is resolved through frictional contact conditions. The proposed method is verified using analytical predictions. The influence of surface energy anisotropy and loading conditions on the resulting crack paths is assessed through a set of benchmark problems. Comparisons are made with the standard Phase Field Finite Element Method and experimental observations.

==> BCBI.tex <==
\subsection{Box-Cantilever beam Impact fracture problem} \label{lbl:BCBI}

In the second example, a box-cantilever beam impact fracture problem is examined. The geometry and boundary conditions are presented in Fig. \ref{fig:BCBI_GeometryBCs}. Initially, a set of parametric study is carried out to investigate the influence of both grid spacing $h$ and length scale parameter $l_0$ on the fracture energy results, comparing them with the analytical solution (ideal fracture). Next, the efficiency of Phase-Field Material Point Method is demonstrated by analysing the post-failure response of that problem. Quadratic b-splines ( $C^{1}$ ) are utilized for the background grid with cell (patch) spacing $h=1.00$ mm, $h=0.50$ mm, $h=0.25$ mm and $h=0.125$ mm. Plain stress conditions are also assumed with thickness $2$ mm. Two discrete fields are considered in this example, namely A for the box(impactor) and B for the cantilever beam(target) with friction coefficient $\mu_{f}=2.00$ between them. The explicit time integrator is used for the solution procedure with timestep $\Delta t = 0.0125$ $\mu$s. An initial velocity is applied to all material points in the box $\dot{\mathbf{u}}_{Ap_{(0)}}=0.02$ mm/$\mu$s and the self-weight of both the box and the cantilever beam is taking into account. The second order isotropic model is considered for that problem, therefore $\gamma_{ijkl} = 0$. The surface energy density of the beam is considered sufficiently large (i.e. $\mathcal{G}_{c_{A}} \left( \theta \right) =1000$ N/mm), thus no damage can occur in it. All the simulation parameters are presented in Table \ref{table:BCBI_SimulationParameters}.

\begin{figure}
	\centering
	\includegraphics[width=0.60\columnwidth]{BCBI_GeoBCs.png}
	\caption[]{Box-Cantilever beam impact fracture problem: Geometry and boundary conditions.}
	\label{fig:BCBI_GeometryBCs}
\end{figure}

		
\begin{center}
	\begin{table}
		\begin{small}
			\resizebox{\columnwidth}{!}{\begin{tabular}{ C{1.0cm} C{1.0cm} C{1.0cm} C{1.0cm} | C{2.0cm}  C{5cm} C{5cm} C{1.0cm}  }
					\hline
					\multicolumn{8}{c}{\textbf{Material Parameters}} \\
					\hline
					\multicolumn{4}{c}{Elastic Material Properties} & \multicolumn{4}{c}{Fracture Material Properties} \\    
					\hline
					& \textbf{\underline{A}} & \textbf{\underline{B}}  &   &    &  \textbf{\underline{A}}  & \textbf{\underline{B}}  &  \\
					$E$ & 190000 & 190000  & [N/mm\textsuperscript{2}] & $\gamma_{ijkl}$  & 0.00  & 0.00  & [--]   \\
					$\nu$     & 0.30 & 0.30  & [--] & $l_0$ & 1.00, 0.50, 0.25, 0.125 & 1.00, 0.50, 0.25, 0.125 & [mm]   \\
					$\rho$    & 8000 & 8000 & [kg/m\textsuperscript{3}]  & $k$  & 0.00  & 0.00  & [--] \\
					& & &  & $\mathcal{G}_{c} \left( \theta \right)=\bar{\mathcal{G}}_c$  & 1000.0 & 6.00  & [N/mm] \\
					\hline
					\multicolumn{8}{c}{\textbf{Material Point Method Model}} \\
					\hline
					\multicolumn{5}{l}{$q_{\xi}=q_{\eta}$}          & 2nd   &  &   \\
					\multicolumn{5}{l}{Initial Cell density}        & 3x3   &  &  \\
					\hline
					\multicolumn{8}{c}{{$h$ = 1.00 mm }} \\
					\hline
					\multicolumn{5}{l}{Number of Control Points}    & 11224    &  &  \\
					\multicolumn{5}{l}{Number of Cells   (Patches)} & 120x90=10800    & & \\
					\multicolumn{5}{l}{$\Xi$}                       & $\{0,0,0,0.00833,0.0167,...,0.9833,0.9917,1,1,1\}$     &  &  \\
					\multicolumn{5}{l}{$H$}                         & $\{0,0,0,0.01111,0.0222,...,0.9777,0.9888,1,1,1\}$     &  &  \\
					\multicolumn{5}{l}{Number of Material Points}    & 6300    &  &  \\
					\hline
					\multicolumn{8}{c}{{$h$ = 0.50 mm }} \\
					\hline
					\multicolumn{5}{l}{Number of Control Points}    & 44044    &  &  \\
					\multicolumn{5}{l}{Number of Cells   (Patches)} & 240x180=43200    & & \\
					\multicolumn{5}{l}{$\Xi$}                       & $\{0,0,0,0.004166,0.008333,...,0.991666,0.995833,1,1,1\}$     &  &  \\
					\multicolumn{5}{l}{$H$}                         & $\{0,0,0,0.005555,0.011111,...,0.988888,0.994444,1,1,1\}$     &  &  \\
					\multicolumn{5}{l}{Number of Material Points}    & 25200    &  &  \\
					\hline
					\multicolumn{8}{c}{{$h$ = 0.25 mm }} \\
					\hline
					\multicolumn{5}{l}{Number of Control Points}    & 174484    &  &  \\
					\multicolumn{5}{l}{Number of Cells   (Patches)} & 480x360=172800    & & \\
					\multicolumn{5}{l}{$\Xi$}                       & $\{0,0,0,0.002083,0.004166,...,0.995833,0.997916,1,1,1\}$     &  &  \\
					\multicolumn{5}{l}{$H$}                         & $\{0,0,0,0.002777,0.005555,...,0.994444,0.997222,1,1,1\}$     &  &  \\
					\multicolumn{5}{l}{Number of Material Points}    & 100800    &  &  \\					
					\hline
					\multicolumn{8}{c}{{$h$ = 0.125 mm }} \\
					\hline
					\multicolumn{5}{l}{Number of Control Points}    & 694564    &  &  \\
					\multicolumn{5}{l}{Number of Cells   (Patches)} & 960x720=691200    & & \\
					\multicolumn{5}{l}{$\Xi$}                       & $\{0,0,0,0.001041,0.002083,...,0.997916,0.998958,1,1,1\}$     &  &  \\
					\multicolumn{5}{l}{$H$}                         & $\{0,0,0,0.001388,0.002777,...,0.997222,0.998611,1,1,1\}$     &  &  \\
					\multicolumn{5}{l}{Number of Material Points}    & 403200    &  &  \\					
					\hline
					\multicolumn{8}{c}{\textbf{Discrete Fields}} \\
					\hline
					\multicolumn{5}{l}{Number of Discrete Fields}             & 2   &  & \\					
					\multicolumn{5}{l}{$\mu_{f}$}             & 2.00   &  & \\					
					\hline
					\multicolumn{8}{c}{\textbf{Solution Algorithm Parameters}} \\
					\hline
					\multicolumn{5}{l}{Time Integrator}             & Explicit  &  & \\
					\multicolumn{5}{l}{$\Delta t$}                  & 0.0125     &  & [$\mu$s] \\
					\multicolumn{5}{l}{$N_{staggs}$}                & 1         &  &  \\
					\hline
				\end{tabular}}
			\end{small}
			\caption{Box-Cantilever beam impact fracture problem: Simulation parameters.}
			\label{table:BCBI_SimulationParameters}
		\end{table}
	\end{center}	



